Range Reporting for Time Series via Rectangle Stabbing

We study the Fr\'echet queries problem. It is a data structure problem, where we are given a set $S$ of $n$ polygonal curves and a distance threshold $\rho$. The data structure should support queries with a polygonal curve $q$ for the elements of $S$, for which the continuous Fr\'echet distance to $q$ is at most $\rho$. Afshani and Driemel in 2018 studied this problem for two-dimensional polygonal curves and gave upper and lower bounds on the space-query time tradeoff. We study the case that the ambient space of the curves is one-dimensional and show an intimate connection to the well-studied rectangle stabbing problem. Here, we are given a set of hyperrectangles as input and a query with a point $q$ should return all input rectangles that contain this point. Using known data structures for rectangle stabbing or orthogonal range searching this directly leads to a data structure with $\mathcal{O}(n \log ^{t-1} n)$ storage and $\mathcal{O}(\log^{t-1} n+k)$ query time, where $k$ denotes the output size and $t$ can be chosen as the maximum number of vertices of either (a) the stored curves or (b) the query curves. The resulting bounds improve upon the bounds by Afshani and Driemel in both the storage and query time. In addition, we show that known lower bounds for rectangle stabbing and orthogonal range reporting with dimension parameter $d= \lfloor t/2 \rfloor$ can be applied to our problem via reduction. .

==> relatedwork_old.tex <==
\paragraph{Related Work.} 
Different data structures are known to solve variants of the \FQ problem. In the following, we review some of them. Let $n$ denote the number of stored curves, $t_s$ the complexity of the stored curves and $t_q$ the complexity of the query curve $q$. \\
The approximation version of the \FQ problem has been widely studied \cite{DP21,DS17,EP20, FFK20,Ind02}. For the discrete \Fm, the $(1+\epsilon)$-ANN data structure by Filtser, Filtser and Katz has size $n\cdot \mathcal{O}\left(1/\varepsilon\right)^{t_{q} d}$ and has query time in $\mathcal{O}(t_{q} d)$, where $d$ is the dimension of the curves \cite{FFK20}.\\ 
However, for the continuous \Fm, it seems to be more challenging to resolve this problem. In a recent work, Bringmann et al. \cite{BDNP21} studied this problem for one-dimensional curves. They improved upon some results of Driemel and Psarros \cite{DP21}. In both papers, the concept of \emph{signatures} and \emph{straightenings} is used, which provides useful features. 
Using a bucketing method, they construct a relatively small set of curves $S'$ depending on the input curves $S$, which are stored in a dictionary. Given a query curve $q$, there must exist a curve in $S'$ very close to $q$ if there exists some curve in $S$ within distance $\rho$ of $q$. In this way, they constructed a $(1+\varepsilon)$-ANN data structure of size $n\cdot\mathcal{O}(t_s/(t_q\varepsilon))^{t_q}$ and query time in $\mathcal{O}(1)^{t_q}$. The query time reduces to $\mathcal{O}(t_q)$ with the same space bound for the $(2+\varepsilon)$-ANN data structure. Furthermore, a $(2+\varepsilon)$-ANN data structure with linear size $\mathcal{O}(t_s n)$ and query time in $\mathcal{O}(1/\varepsilon)^{t_q+2}$ is obtained. In addition, they present conditional lower bounds for several different settings of the problem based on the Orthogonal Vectors Hypothesis.\\
Afshani and Driemel \cite{AfshaniDriemel18} studied the Fréchet queries problem in 2018 for both the discrete and the continuous \Fm. In contrast to the $c$-ANN, all curves within distance $\rho$ from a query curve $q$ must be reported. They show how to build multi-level partition trees for two-dimensional curves using semi-algebraic range searching, which can be used to solve the \FQ problem. This data structure has size $\mathcal{O}\left(n (\log\log n)^{\mathcal{O}({t_s}^2)}\right)$ and uses query time in $\mathcal{O}\left(\sqrt{n}\cdot \log^{\mathcal{O}({t_s}^2)}n\right)$. Obviously, this data structure can also be used to solve the problem for one-dimensional curves. Here, orthogonal range searching can be used. In this case, their bounds reduce to $\mathcal{O}\left(n\left({\log n}/{\log \log n}\right)^{\mathcal{O}({t_s}^2)}\right)$ size and $\mathcal{O}\left(\log n\cdot \left({\log n}/{\log \log n}\right)^{\mathcal{O}({t_s}^2)}\right)$ query time in the one-dimensional case.
They store for all time series $s$ of complexity at most $t_s$ an $\mathcal{O}({t_s}^2)$-dimensional point $p(s)$. The dimension of $p(s)$ is quadratic in $t_s$, because for every pair of vertices of $s$ values depending on both vertices are stored.
Additionally, using a volume argument they provide a lower bound in the pointer machine model, stating that every data structure with $Q(n) +\mathcal{O}(k)$ query time, where $k$ is the output size, has to use roughly $\Omega((n/Q(n))^2)$ space in the worst case even if the query curves are just line segments or points for the discrete \Fm.


